Faster Algorithms for Growing Collision-Free Convex Polytopes in Robot Configuration Space

We propose two novel algorithms for constructing convex collision-free polytopes in robot configuration space. Finding these polytopes enables the application of stronger motion-planning frameworks such as trajectory optimization with Graphs of Convex Sets [1] and is currently a major roadblock in the adoption of these approaches. In this paper, we build upon IRIS-NP (Iterative Regional Inflation by Semidefinite & Nonlinear Programming) [2] to significantly improve tunability, runtimes, and scaling to complex environments. IRIS-NP uses nonlinear programming paired with uniform random initialization to find configurations on the boundary of the free configuration space. Our key insight is that finding near-by configuration-space obstacles using sampling is inexpensive and greatly accelerates region generation. We propose two algorithms using such samples to either employ nonlinear programming more efficiently (IRIS-NP2 ) or circumvent it altogether using a massively-parallel zero-order optimization strategy (IRIS-ZO). We also propose a termination condition that controls the probability of exceeding a user-specified permissible fraction-in-collision, eliminating a significant source of tuning difficulty in IRIS-NP. We compare performance across eight robot environments, showing that IRIS-ZO achieves an order-of-magnitude speed advantage over IRIS-NP. IRISNP2, also significantly faster than IRIS-NP, builds larger polytopes using fewer hyperplanes, enabling faster downstream computation. Website: https://sites.google.com/view/fastiris

==> body/bernoulli_new.tex <==
\section{Bernoulli New}
\newcommand{\Bern}{\mathrm{Bernoulli}}
\subsection{A nonadaptive test}
\begin{lemma}[Bernoulli Multiplicative Concentration]\label{lem:Bern_conc} Let $(X_i)_{i \ge 1} \sim \mathrm{Bernoulli}(p)$, and let $N$ be fixed. Define $\bar X_N := \frac{1}{N}\sum_{i=1}^N X_i$. Then, for any fixed parameter $\tau > 0$
\begin{align}
    \Pr\left[\bar X_N  \ge (1+\tau) p \right] \le e^{-Np\tau^2/(2+\tau)}.
\end{align}
Moreover, if $0 < \tau \le 1$, 
\begin{align}
    \Pr\left[\bar X_N  \le (1-\tau) p \right] \le e^{-Np\tau^2/2}.
\end{align}
\mscomment{source: wikipedia}
\pwcomment{ \href{https://en.wikipedia.org/wiki/Chernoff_bound}{link}}

\end{lemma}
As a consquence of the second part of the lemma, we obtain the corrolary:
\begin{corollary} Let $(X_i)_{i \ge 1} \sim \mathrm{Bernoulli}(p')$, $p' \ge p$. Then, 
\begin{align}
    \Pr\left[\bar X_N  \le (1-\tau) p \right] \le e^{-Np\tau^2/2}.
\end{align}
Hence, with $N = 2\log(1/\delta)/p\tau^2$ samples, I have that if $(X_i)_{i \ge 1} \sim \mathrm{Bernoulli}(p')$, $p' \ge p$,
\begin{align}
    \Pr[ \bar X_N \le (1-\tau)p ] \le \delta. 
\end{align}
\end{corollary}
\textbf{Proof}
    $\Pr\left[\bar X_N  \le (1-\tau) p \right] \le \Pr\left[\bar X_N  \le (1-\tau) p' \right]  \le e^{-Np'\tau^2/2} \le  e^{-Np\tau^2/2}$. The second result follows by evaluation. \qed
\newcommand{\pdes}{p_{\mathrm{des}}}


From this Lemma, let us consider the following procedure.
\begin{definition}\label{def:unadaptive_test} Let $\mathsf{UndaptiveTest}(N,p,\tau)$ collect $N$ samples $(X_i)_{1 \le i \le N}$. We ``reject'' if $\bar{X}_N > (1-\tau)p$, and accept otherwise.
\end{definition}
\begin{corollary} Suppose that $(X_i)_{1 \le i \le N} \sim \mathrm{Bernoulli}(p')$, $p' \ge p$. Then,  $\mathsf{UndaptiveTest}(N,p,\tau)$ rejects with probability at least $1 - \delta$ for $N = \frac{2 \log(1/\delta)}{p \tau^2}$. 
\end{corollary}
\pwcomment{Just writing out the proof so we dont get anything wrong}

\textbf{Proof}
\begin{align}
\Pr[\bar{X}_N>(1-\tau)p'] = 1 - \Pr[\bar{X}_N\leq(1-\tau)p']\geq1-\delta     
\end{align}
\qed
So far, we have only controlled the type II error of false accept. The following lemma also controls the power of accepting. 
\begin{lemma} Fix $\tau,\tau_- > 0$. $(X_i)_{i \ge 1} \sim \Bern(p')$, $p' \le \tilde{p} := \frac{(1-\tau)}{1+\tau_- }\cdot p$. Then, $\Pr[\bar{X}_N \ge (1-\tau)p] \le e^{-Npc}$, $c = \frac{\tau_-^2(1-\tau)}{(2+\tau_-)(1+\tau_-)}.$  
\end{lemma}
\textbf{Proof}. It is easy to see that $\bar{X}_N$ is stochastically dominated by $\bar{\tilde X}_N := \frac{1}N\sum_{i=1}^N \tilde X_i$ is the average of $N$ i.i.d. drawns from Bernoulli $\tilde{p}$. Hence, it suffices to prove the lemma when $p' = \tilde p $. In this case, using the definition of $\tilde{p}$ and invoking \Cref{lem:Bern_conc},
\begin{align}
    \Pr[\bar{X}_N \ge (1-\tau)p] &= \Pr\left[\bar X_N  \ge (1+\tau_-) \tilde{p} \right] \le 
    e^{-Np\tau_-^2/(2+\tau_-)} \\
    &=  e^{-N pc} 
\end{align}

which concludes the proof. \qed 
\newcommand{\UnadapTest}{\mathsf{UndaptiveTest}}
\begin{proposition} Fix $\tau, \tau_- \in (0,1)$, $p \in (0,1)$, and let  
\begin{align}
N = N(p,\delta, \tau, \tau_-) := \frac{1}{p}\log(1/\delta) \max\left\{\frac{2}{\tau^2}, \frac{(2+\tau_-)(1+\tau_-)}{\tau_-^2(1-\tau)}\right\}
\end{align}
samples. Let $(X_i)_{i \ge 1} \sim \Bern(p')$. Then, 
\begin{itemize}
    \item[(a)] If $p' \ge p$, $\UnadapTest(N,p,\tau)$ rejects with probability $1 - \delta$.
    \item[(b)] If $p' \le \frac{1-\tau}{1+\tau_-}p$, $\UnadapTest(N,p,\tau)$ accepts with probability at least $1 - \delta$.
\end{itemize}
\end{proposition}

\pwcomment{I find the $\tau_-$ very unintuitive. I see that it controls the sample  count if we want more accepting power. In practice if I impose a $\tau$ then there should be a smallest $\tau_-$ such that $N$ doesnt increase, why not just use that?}

\begin{definition}[Sequential Test] Fix parameters $p,\delta,\tau,\tau_-$. Define 
\begin{align}
\delta_k := \delta \cdot \frac{6}{\pi^2k^2}.
\end{align} At iteration $k$ of the algorithm, you run $\UnadapTest(N_k,p,\tau)$, where $N_k = N(p,\delta_k,\tau,\tau_-)$. 
    
\end{definition}

\begin{corollary} Consider a sequence of random variables $(X_{k,i})_{k, 1 \le i \ge N_i}$. Suppose that, conditioned on $s$
\end{corollary}


\subsection{An adaptive Test }
\begin{definition}
    Given $N \in \mathbb N$ and $k \le \log_2 N$, define 
\end{definition}

\newcommand{\KL}{\mathrm{KL}}
\newcommand{\kl}{\mathrm{kl}}
\newcommand{\iidsim}{\overset{i.i.d.}{\sim}}
\subsection{And now for something different (KL Confidence Interval)}

Sharper Chernoff
\begin{align}
    \Pr[\bar X_N \le (1-\tau)p] \le \exp(-pN \left(\tau - (1-\tau)\log(1-\tau)\right)) 
\end{align}
Hence, for 
\begin{align}
    N \ge \frac{\log (1/\delta)}{p\left(\tau + (1-\tau)\log(1-\tau))\right) },
\end{align}
we have $\Pr[\bar X_N \le (1-\tau)p] \le \delta$. Define $c_{\tau} := left(\tau + (1-\tau)\log(1-\tau)) $For $\tau = .5$, we get 
\begin{align}
    c_
\end{align}






==> body/bernoulli_trial_old.tex <==
\section{Bernoulli Trial Discussion}

We want to terminate as soon as it holds that 
\begin{gather}\label{eq:terminationproblem}
\Prob\Big(\frac{\lambda(\calR\cap\Cfree)}{\lambda(\calR)}\geq 1-\varepsilon\Big) \geq \alpha,
\end{gather}
where $\lambda$ denotes the Lebesgue measure in $\Cfree$, $\calR$ denotes our collision free set, $\varepsilon$ is the admissible fraction of the volume in collision and $\alpha$ is the certainty threshold.

\textbf{The following is rearranging arguments in \cite{yang2004sampling} for their termination condition and applying it to our setting. }

Let $Y$ be a random variable, corresponding to a configuration uniformly drawn in $\calR$. The variable $Y$ takes the value 0 if the configuration is collision-free, and 1 if it is in collision. The variable $Y$ therefore has a Bernoulli distribution with 
\begin{gather}
    \Prob(Y=0)=\theta \text{ and } \Prob(Y=1)=1-\theta, 
\end{gather}
where 
\begin{gather}    
\theta = \frac{\lambda(\calR\cap\Cfree)}{\lambda(\calR)}
\end{gather}

We can use trials of $Y$ to estimate $\theta$. Let $Y_1, Y_2, \dots ,Y_m$ be a sequence of independent trials, and $\bar Y$ be the sample mean. (Note that $\bar Y$ is an unbiased estimator of $\theta$.)

For a given $\varepsilon$ and given a decision threshold $T\in(0,1)$ (more on that later), the probability $\alpha$ (the \textit{confidence level}), that $1-\bar Y \geq T$, implies $\theta\geq1-\varepsilon$ is

\begin{gather}
    \alpha = 1-(1-\varepsilon)^{m+1}\sum^{\lfloor m(1-T)\rfloor}\begin{pmatrix}
        m\\i
    \end{pmatrix}\Big(\frac{1}{(1-\varepsilon)^i(m-i+1)}- \frac{1}{m+1}\Big).
\end{gather}

\textit{proof}: Rejecting the null hypothesis when it is true is called a type $I$ error. In our case this would correspond to $1-\bar Y<T$ even though it holds that $\theta\geq 1-\varepsilon$. (Think: Too many collisions increases the value of $\bar Y$ even though it should be lower, due to the high probability - or $\theta$ - of drawing a 0.) Falsely accepting the null  hypothesis when it is false is called a type $II$ error. In our case this corresponds to the estimated free volume being above the acceptance threshold even though the actual free volume is below it; $1-\bar Y\geq T$ even though we have $\theta< 1-\varepsilon$. (Note $\alpha = 1- \Prob(\text{type } II \text{ error})$).

Let $X$ denote a random variable corresponding to the number of samples in collision $k$ for $m$ trials. The variable $X$ has a binomial distribution

\begin{gather}
    \Prob(X=k) = \begin{pmatrix}
        m\\k
    \end{pmatrix}\theta^{m-k}(1-\theta)^k,
\end{gather}

thus, 
\begin{align}
   \Prob(1-\bar Y\geq T; ~\theta< 1-\varepsilon)\\
    =&\Prob(X\leq \lfloor m(1-T) \rfloor; ~\theta< 1-\varepsilon)\\
    =&\int_0^{1-\varepsilon}\sum_{i=0}^{\lfloor m(1-T) \rfloor}\begin{pmatrix}
        m\\i
    \end{pmatrix}\theta^{m-i}(1-\theta)^id\theta\\
    =&\sum_{i=0}^{\lfloor m(1-T) \rfloor}\begin{pmatrix}
        m\\i
    \end{pmatrix}\int_0^{1-\varepsilon}\theta^{m-i}\sum_{j = 0}^i\begin{pmatrix}
        i\\j
    \end{pmatrix}(-1)^{j}\theta^jd\theta\\
    =&\sum_{i=0}^{\lfloor m(1-T) \rfloor}\begin{pmatrix}
        m\\i
    \end{pmatrix}\int_0^{1-\varepsilon}\sum_{j = 0}^i\begin{pmatrix}
        i\\j
    \end{pmatrix}(-1)^{j}\theta^{m-i+j}d\theta\\
    =&\sum_{i=0}^{\lfloor m(1-T) \rfloor}\begin{pmatrix}
        m\\i
    \end{pmatrix}\sum_{j = 0}^i\begin{pmatrix}
        i\\j
    \end{pmatrix}(-1)^{j}\int_0^{1-\varepsilon}\theta^{m-i+j}d\theta\\
    =&\sum_{i=0}^{\lfloor m(1-T) \rfloor}\begin{pmatrix}
        m\\i
    \end{pmatrix}\sum_{j = 0}^i\begin{pmatrix}
        i\\j
    \end{pmatrix}(-1)^{j}\frac{1}{m-i+j+1}(1-\varepsilon)^{m-i+j+1},
\end{align}
I am stuck with the integral here -> either do integration by parts at step (8) or resolve this sum

An alternative perspective is, consider drawing $m$ samples in succession, $Y_1, \dots, Y_m$, and the first collision happens at the $m$-th sample.
Let $M>0$ be a termination threshold, and $X$ be a random variable that corresponds to the number of trials until the first collision is found.
The probability of making an error of the second kind, i.e. the probability that $m\geq M$ even though $\theta<1-\varepsilon$ is
\begin{gather}
    \Prob(X\geq M ; \theta<1-\varepsilon)\\
    \underbrace{=}_{X\sim\text{geom. }}\int_0^{1-\varepsilon}\Prob(X\geq M)d\theta\\
    = \int_0^{1-\varepsilon} 1 - \Prob(X< M)d\theta\\
    = \int_0^{1-\varepsilon} 1- \sum_{m 
 = 1}^{M-1}\theta^{m-1}(\theta -1)d\theta\\
 = \Big[\theta + \sum_{m 
 = 1}^{M-1}\frac{\theta^{m+1}}{m+1} - \frac{\theta^{m}}{m}\Big]^{1-\varepsilon}_0\\
 =\frac{(1-\varepsilon)^M}{M},
\end{gather}
which implies that 
\begin{gather}
    \Prob(X\geq M ; \theta\geq1-\varepsilon) = 1-\frac{(1-\varepsilon)^M}{M}.
\end{gather}

Therefore, if we want (\ref{eq:terminationproblem}) to hold, we need 
\begin{gather}
    \alpha\leq1-\frac{(1-\varepsilon)^M}{M}.\\
\end{gather}
We can derive a tighter bound in closed form as follows
\begin{gather}
\alpha\leq 1-(1-\varepsilon)^M\leq1-\frac{(1-\varepsilon)^M}{M}\\
\Leftrightarrow M\geq \frac{\log(1-\alpha)}{\log(1-\varepsilon)} -1.
\end{gather}

\newpage

\begin{gather}
    \sum_{j = 0}^i\begin{pmatrix}
        i\\j
    \end{pmatrix}(-1)^{j}\frac{1}{m-i+j+1}(1-\varepsilon)^{m-i+j+1}
\end{gather}

\pwcomment{Not done but likely not necessary}

\section{Old Approach using Normal Approximation of Binomial Distribution}

Let $(X_i)_{i \ge 1} \sim \mathrm{Bernoulli}(p)$, and let $N$ be fixed. Define $Y_N :=\sum_{i=1}^N X_i$. The random variable $Y$ is binomially distributed with $Y\sim\mathrm{Binomial}(N,p)$. Let $Z\sim\calN\Big(Np, \sqrt{Np(1-p)}\Big)$. Then for a threshold $T\inR$, by the Berry-Esseen theorem, 
\begin{align}
    \Pr(Y\leq T)\approx\Pr(Z\leq T) = \Phi\Bigg(\frac{T-Np}{\sqrt{Np(1-p)}}\Bigg),
\end{align}

 as the sample count $N$ tends towards infinity. The function $Phi$ denotes the normal cumulative distribution function. As a rule of thumb, the approximation is considered good if $Np(1-p)\geq10$ {\color{red}source math stack exchange, this sets the sup of the differences of the pdf to $\sim$ 0.15}.

Now, let $p'\geq p$, and $Z\sim\calN\Big(Np, \sqrt{Np(1-p)}\Big)$ as well as $Z'\sim\calN\Big(Np', \sqrt{Np'(1-p')}\Big)$. It holds that 
\begin{align}
    \Pr[Z\leq T]\leq \Pr[Z' \leq T] = \Phi\Bigg(\frac{T-Np'}{\sqrt{Np'(1-p')}}\Bigg) \leq\Phi\Bigg(\frac{T-Np}{\sqrt{Np(1-p)}}\Bigg)
\end{align}

We get the last inequality by the monotonicity of $\Phi$ and observing that
\begin{align}
    \frac{d}{dp} \frac{T-Np}{\sqrt{Np(1-p)}} = -\frac{N(Np-2Tp+T)}{2(N(1-p)p)^{3/2}}
\end{align}

is nonpositive for $0<p<1$, assuming $T\leq N$. These assumptions make the denominator positive and the result follows from $Np-2Tp+T\geq p(N-T)\geq0$.\qed

We can now design our test. Assume $p'\geq p$ we collect N samples and the number of samples in collision $Y\leq T$ we want to control the probability of falsely accepting our null hypothesis when it is not true. We accept a $\delta>0$ error probability. Let 

\begin{align}
    T = \Phi^{-1}(\delta)\sqrt{Np(1-p)} + Np.
\end{align}

If $Z\sim\calN\Big(Np', \sqrt{Np'(1-p')}\Big)$, then the test rejects with at least probability $1-\delta$. We obtain the result by plugging in

\begin{align}
    \Pr[Z\leq T] &=\Phi\Bigg(\frac{T-Np'}{\sqrt{Np'(1-p')}}\Bigg)\\
    &\leq \Phi\Bigg(\frac{T-Np}{\sqrt{Np(1-p)}}\Bigg)\\
    &= \delta,
\end{align}

therefore
\begin{align}
     \Pr[Z>T] = 1 -\Pr[Z\leq T]\geq 1-\delta. 
\end{align}
\qed

Now need to argue that if $N$ large enough we hold our breaths and say $Z=Y$, which is what I did.

==> body/structure.tex <==

\section{Structure of the paper}
Not much thought has gone into this yet
\begin{itemize}
    \item Introduction
    \item Motivation
    \begin{itemize}
        \item Motion Planning (GCS, FPP, accelerate RRT?, others?)
    \end{itemize}
    \item Related Works
    \begin{itemize}
        \item Iris + ciris + clique seeding
        \item lavalle 
        \item vhacd
        \item taskspace??
    \end{itemize}
    \item Further Background (Section explaining original iris)
    \begin{itemize}
        \item Iris background
        \item Sperating hyperplanes in cspace becomes problematic 
        \item Iris Np idea, drawbacks, probabilistic imprecise, nonlinear optimizer slow, doesnt scale with compute 
        \item TODO: discuss step-back (``less absolute volume in collision'' -- note that relative could go up or down)
    \end{itemize}
    \item Approximating the Separating planes step
    \begin{itemize}
        \item Guiding principle: we can check if an individual sample is in collision super super super duper quickly. So if we draw tons of samples, we can leverage that to speed up these algorithms. We will search for regions with a certain proportion not in collision, so the curse of dimensionality does not present an obstacle
        \item Define Finding closest point in collision program
        \item Describe the batch structure, and how it lets us terminate. (Include the fancy derived termination condition, and stick the derivation in the appendix. Note that this is true for any black box algorithm which constructs hyperplanes.)
        \item Specific optimization methods
        \begin{itemize}
            \item FastIris
            \item GreedyIris
            \item RayIris
        \end{itemize}
    \end{itemize}
    \item Numerical Experiments
    \begin{itemize}
        \item run benchmarks for various settings
        \item how calibrate settings?
    \end{itemize}
    \item Conclusion
\end{itemize}

==> data/table.tex <==
\begin{table}
\centering
\begin{minipage}{1\linewidth}
        \resizebox{\linewidth}{!}{

\begin{tabular}{c l cccc | cccc | cccc | cccc}
\hline
\multirow{2}{*}{}&\multirow{2}{*}{Environment}& \multicolumn{4}{c}{Time [s]} & \multicolumn{4}{c}{Num Hyperplanes} & \multicolumn{4}{c}{Rel Volume} & \multicolumn{4}{c}{Frac in collision} \\
 &&NP& Fast & Greedy& Ray & NP & Fast& Greedy & Ray & NP& Fast & Greedy & Ray& NP& Fast & Greedy & Ray \\
\hline
\multirow{8}{*}{\rotatebox[]{90}{\textbf{Fast}}\;} 
&\texttt{Flipper} &
0.168& 0.0252& 0.0451& 0.847& 22.7& 15.8& 13.6& 13.4& 1& 0.627& 2.17& 2.02& 0.0396& 0.0131& 0.0218& 0.0161\\
&\texttt{UR3} &
0.994& 0.041& 0.113& 0.221& 41.6& 27.8& 25.4& 22.7& 1& 0.971& 3.6& 3.3& 0.0404& 0.0286& 0.0203& 0.0281\\
&\texttt{UR3Wrist} &
1.23& 0.0496& 0.168& 0.948& 51.4& 34& 30.8& 26.5& 1& 3.82& 5.38& 1.66& 0.0285& 0.0306& 0.0234& 0.0232\\
&\texttt{IIWAShelf} &
1.35& 0.0911& 0.442& 0.633& 77.3& 47.2& 32.7& 31& 1& 6.2& 8.73e+03& 16.2& 0.0678& 0.0343& 0.0274& 0.0519\\
&\texttt{4Shelves} &
1.32& 0.0921& 0.313& 0.845& 62.9& 46.9& 35.1& 30.3& 1& 0.139& 1.39& 1.72& 0.102& 0.0376& 0.0248& 0.0328\\
&\texttt{IIWABins} &
1.54& 0.0744& 0.627& 0.861& 84& 44.3& 33.4& 31.1& 1& 542& 4.99e+04& 604& 0.0922& 0.0354& 0.0271& 0.0209\\
&\texttt{2IIWAs} &
20.5& 2.02& 62.1& 46.5& 242& 246& 77.7& 65.7& 1& 0.000805& 317& 95.1& 0.0606& 0.0567& 0.0375& 0.0554\\
&\texttt{Allegro} &
2.28& 0.264& 0.101& 0.106& 75.3& 83.7& 41.9& 39.6& 1& 0.0357& 152& 60.6& 0.000684& 0.0522& 0.0147& 0.0331\\
\hline
\multirow{8}{*}{\rotatebox[]{90}{\textbf{Precise}}\;} 
&\texttt{Flipper} &
1& 0.172& 0.152& 0.269& 26.1& 17.8& 14.3& 14.4& 1& 0.621& 1.17& 1.24& 0.00297& 0.00107& 0.00104& 0.000402\\
&\texttt{UR3} &
5.22& 0.304& 0.325& 0.642& 52.9& 44.5& 28.1& 27& 1& 3.7& 13.7& 2.3& 0.00306& 0.00214& 0.00205& 0.00337\\
&\texttt{UR3Wrist} &
4.66& 0.359& 0.359& 0.41& 61.8& 56.1& 31.5& 28.6& 1& 3.81& 183& 4.96& 0.00203& 0.00262& 0.00131& 0.00178\\
&\texttt{IIWAShelf} &
11.3& 0.787& 1.09& 3.01& 126& 92& 41& 37.8& 1& 764& 7.82& 9.26& 0.00409& 0.00314& 0.00183& 0.00381\\
&\texttt{4Shelves} &
25.3& 0.699& 0.838& 1& 85.2& 81.3& 40.5& 36.1& 1& 0.124& 1.59& 1.67& 0.0125& 0.00285& 0.00159& 0.00272\\
&\texttt{IIWABins} &
15.5& 0.763& 0.997& 2.19& 129& 98.6& 44.1& 39.6& 1& 504& 603& 92.3& 0.00348& 0.0031& 0.00164& 0.00311\\
&\texttt{2IIWAs} &
203& 43.2& 85& 77.2& 395& 739& 90.8& 82.7& 1& 0.000278& 37.5& 49& 0.00551& 0.00498& 0.00357& 0.00398\\
&\texttt{Allegro} &
2.16& 7.45& 0.499& 1.27& 75.3& 291& 45.5& 42.2& 1& 0.00539& 8.24& 20.4& 0.000736& 0.00473& 0.00134& 0.00302\\
\hline
\end{tabular}
}
\end{minipage}
\caption{Statistics averaged over all 10 seed points.  ``Rel Volumes'' are polytope maximimum-volume inscribed ellipsoid volumes, normalized by that of IRIS-NP.}
\label{tab:results}
\end{table}

==> figures/benchmarks/data/fast_iris_balanced.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
0.05410353183746338	0.074576020741906	0.00419	17.05	0.02171699047088623	0.07341241439601431	0.00419	6.050000000000001	0.08426626682281493	0.16155026355118857	0.03341	8.95	1
0.06915605545043946	0.010151243533121475	0.011302000000000001	36.56	0.03474319458007813	0.0101510528902003	0.010702000000000001	20.560000000000002	0.08705484390258789	0.04857944268265373	0.022098	37.44	2
0.07896869659423827	0.002094810814481507	0.013074	46.69	0.036048822402954095	0.0020948064916892126	0.011074	21.689999999999998	0.07540423393249512	0.02245188487576684	0.015926000000000003	24.310000000000002	3
0.1357942533493042	0.00243439253185248	0.01505	81.14	0.05755528926849365	0.0024343925304983797	0.01445	51.14	0.09222426891326904	0.023993201596542377	0.018349999999999998	145.86	4
0.15393616914749145	4.272962875583697e-06	0.015398	72.83	0.06649400949478149	4.272955369272957e-06	0.014198	38.83	0.11242292165756226	3.5486981698036236e-05	0.015201999999999999	89.17	5
0.11604185819625855	0.005997815900489659	0.016597999999999998	80.81	0.059180696010589603	0.00599781584908923	0.015998	46.81	0.09047202348709106	0.05809630500643665	0.020002000000000002	198.19	6
7.723146078586578	3.492348842370861e-13	0.02628	1487.93	7.13769376039505	3.4923488423658827e-13	0.01908	1325.93	57.17542922735214	6.182644601457637e-12	0.012719999999999999	5965.07	7
0.6155493640899659	2.1887858718183148e-10	0.023794	260.76	0.5371778392791748	2.1887858455294714e-10	0.019794	224.76	2.224719009399414	3.1837949809334945e-09	0.035206	691.24	8


==> figures/benchmarks/data/fast_iris_balanced_3.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
0.06219057559967041	0.0747102087610323	0.003538	17.08	0.023988289833068846	0.07358751107883357	0.003538	6.079999999999998	0.07986302852630615	0.16534680780696104	0.022262	6.920000000000002	1
0.07616308212280273	0.010408198175412766	0.011272000000000003	35.41	0.03356125831604004	0.010407992965550722	0.011072000000000002	19.409999999999997	0.08978650093078613	0.06600698580329553	0.024127999999999997	45.59	2
0.09033100843429566	0.0020596100525114066	0.013413999999999999	45.09	0.031315257549285894	0.00205960555694419	0.011413999999999999	18.090000000000003	0.1654115414619446	0.02321567469137584	0.019786	28.909999999999997	3
0.15838372707366943	0.002485083621685145	0.015761999999999998	71.34	0.08438122272491455	0.0024850836188214545	0.015361999999999999	47.34	0.16063034534454346	0.022406206778159368	0.021238	62.66	4
0.187699875831604	4.538212941282501e-06	0.015724000000000002	66.52	0.07679780483245849	4.538207157799581e-06	0.010924000000000003	38.519999999999996	0.18700424671173096	3.65002238066182e-05	0.016276	47.480000000000004	5
0.1312948203086853	0.005709510890854871	0.014822000000000002	70.06	0.06462321043014527	0.005709510846355057	0.014822000000000002	37.06	0.15083256006240844	0.056088420770450315	0.034578	63.94	6
3.7140894889831544	3.794645505043981e-13	0.026860000000000005	495.29	2.9905198574066163	3.7946455050406236e-13	0.012860000000000005	348.29	13.326706314086914	4.863907447660478e-12	0.012739999999999998	1009.71	7
0.5605127811431885	2.441497383112728e-10	0.023897999999999996	174.21	0.4739346504211426	2.4414973636522307e-10	0.023897999999999996	138.21	1.2760050296783447	3.689530492428845e-09	0.03290200000000001	277.78999999999996	8


==> figures/benchmarks/data/fast_iris_fast.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
0.02591740131378174	0.07088630434135211	0.008574	17.0	0.010398020744323732	0.06995364023797175	0.008574	7.0	0.05831492900848388	0.12149975119539443	0.036626	9.0	1
0.038706467151641846	0.012391330965119452	0.021466	33.08	0.013363287448883057	0.01239105119003465	0.019865999999999998	14.079999999999998	0.0701571249961853	0.0738381272616414	0.043534	38.92	2
0.04380267858505249	0.0020046315761927318	0.026475999999999996	43.23	0.013457953929901123	0.0020046253148506598	0.022075999999999995	19.229999999999997	0.059220850467681885	0.021243130468924034	0.034524	21.770000000000003	3
0.0795477271080017	0.003659166964302357	0.034230000000000003	72.85	0.04142888784408569	0.0036591669567705007	0.029630000000000004	48.849999999999994	0.10380808115005494	0.03636956981168148	0.03817	140.15	4
0.08180116891860961	5.747881202185154e-06	0.029346	67.92	0.04034232378005981	5.747874800492894e-06	0.019546	40.92	0.08326125860214234	5.566700158325626e-05	0.03765400000000001	77.08	5
0.0686993956565857	0.008887620500521947	0.03166000000000001	69.89	0.03535131216049195	0.008887620426206843	0.029460000000000007	44.89	0.09280439615249633	0.09540999558851207	0.03893999999999999	143.11	6
3.199643039703369	1.124076191549223e-12	0.053634	1083.86	2.925846719741821	1.1240761915486137e-12	0.020434	1006.8599999999999	26.004391527175905	1.7569086907454555e-11	0.038966	4749.14	7
0.32381520509719847	4.1215776592121143e-10	0.047566	176.61	0.2615452790260315	4.1215776227097123e-10	0.042966	140.61	0.7075597262382507	5.987708879889745e-09	0.09243400000000002	387.39	8


==> figures/benchmarks/data/fast_iris_fast_old.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
0.07422971725463867	0.1300075472935413	0.00498	22.58	0.040628671646118164	0.12895897545436233	0.00498	7.579999999999998	0.0466001033782959	0.25535965733324123	0.024620000000000003	12.420000000000002	1
0.10460169792175293	0.040007112891624855	0.012707999999999999	57.58	0.051541166305541994	0.04000682397331423	0.011508	30.58	0.0976123046875	0.16884688828756472	0.011692000000000003	57.42	2
0.131280837059021	0.020234879854595284	0.015704	85.06	0.0739080286026001	0.020234875788434543	0.011504	48.06	0.08552080631256104	0.08719362223339919	0.015695999999999998	65.94	3
0.2223514747619629	0.012403810055597483	0.016808	153.08	0.15689389228820802	0.012403810052933494	0.012208	128.08	0.40586598396301266	0.09361590976246872	0.012591999999999999	292.91999999999996	4
0.1290101194381714	1.5006944741720938e-05	0.015604	82.76	0.05715123653411866	1.5006939067717086e-05	0.011203999999999999	48.760000000000005	0.20915063381195068	0.00032661905902179575	0.015396	118.24	5
0.2573614454269409	0.02737055984823827	0.018144	180.7	0.20912626743316648	0.02737055979155162	0.013344000000000002	151.7	0.43476649761199954	0.204008894567574	0.019456	213.3	6
7.985684013366699	3.878720837622225e-13	0.02568	1530.2	7.102656459808349	3.878720837617452e-13	0.01088	1277.2	53.052079105377196	3.658665638389433e-12	0.015719999999999998	5426.8	7
0.6408768939971924	2.8107821146770225e-10	0.024267999999999998	283.5	0.5696181106567383	2.810782094635168e-10	0.022267999999999996	249.5	1.3663021278381349	4.206058693850474e-09	0.020732	478.5	8


==> figures/benchmarks/data/iris_np_fast.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
0.1682763910293579	0.1560011125128415	0.039628	22.7	0.05041392803192138	0.14483890529160875	0.039628	6.699999999999999	0.28833190441131595	0.29675782886600166	0.247172	9.3	1
0.9938970136642457	0.016840084428766215	0.04037000000000001	41.6	0.5516846704483033	0.016835392742080728	0.04037000000000001	14.600000000000001	1.0634645891189574	0.11025896632384462	0.30002999999999996	43.4	2
1.2266513967514039	0.007835968778277198	0.028517999999999998	51.38	0.739893879890442	0.007834697551403548	0.028517999999999998	21.380000000000003	1.2288458681106567	0.0629651212632965	0.235082	31.619999999999997	3
1.345428216457367	0.008276777011549132	0.067844	77.28	0.9203765273094178	0.008276769394759135	0.067844	39.28	1.6800196290016174	0.07552372574971784	0.273356	95.72	4
1.3165054798126221	2.804875038898052e-05	0.10184999999999997	62.86	0.5022519111633301	2.800536980636276e-05	0.10184999999999997	21.86	0.8679301261901855	0.00020850030558201116	0.7353500000000001	30.14	5
1.5357209706306458	0.01505195697236538	0.09216799999999999	83.99	0.9603117966651917	0.015051944455821803	0.09216799999999999	40.989999999999995	1.8121188616752624	0.16284891968382964	0.484632	85.01	6
20.482455456256865	2.397808419328959e-10	0.060582000000000004	242.05	15.372804844379424	2.397808418106169e-10	0.059982	147.05	73.61794523000717	3.39869202309717e-09	0.49601799999999996	471.95	7
2.2767344760894774	4.798052460109174e-09	0.000684	75.34	0.8876391696929931	4.7963264859451586e-09	0.000684	25.340000000000003	1.1399170112609864	3.047447349120994e-08	0.009715999999999999	25.659999999999997	8


==> figures/benchmarks/data/iris_np_medium.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
1.490734326839447	0.14346498791030235	0.0	26.09	0.32312797307968144	0.1041781998816412	0.0	8.09	0.6802446961402893	0.1953779388165687	0.0	6.91	1
9.026874392032623	0.011076544262219934	0.00010999999999999999	55.7	4.650727121829986	0.01107297827795676	0.00010999999999999999	23.700000000000003	11.731538207530976	0.0719652255581665	0.00129	84.3	2
12.297900154590607	0.002977534033288558	0.0009499999999999999	70.74	6.422686293125153	0.002976527804607052	0.0009499999999999999	35.739999999999995	12.749935910701751	0.01964941690968403	0.03465	55.260000000000005	3
17.77518509864807	0.004628850521494348	0.00107	132.14	12.35731696128845	0.0046288477465261735	0.00107	81.13999999999999	52.93467141151429	0.03508990601216895	0.02573	319.86	4
13.208080689907074	1.7170658739462605e-05	0.014196	82.32	5.213692586421967	1.7148655867986392e-05	0.014196	29.319999999999993	6.865448553562164	0.00010050967453301219	0.18940400000000002	41.68000000000001	5
16.241048080921175	0.008237836447592727	0.003308	128.6	10.048620922565462	0.008237828543947475	0.003308	55.599999999999994	25.836498754024504	0.09312268481714839	0.061891999999999996	221.4	6
360.4537730073929	6.398039527555432e-11	0.0014480000000000005	431.18	303.9031808233261	6.398039523351386e-11	0.0014480000000000005	290.18	2360.007499709129	8.111947667577657e-10	0.022151999999999998	1186.82	7
24.104202077388763	2.9348803722338777e-09	1e-05	89.45	7.971556947231292	2.9332114381770187e-09	1e-05	36.45	14.813469841480256	1.3775179641833563e-08	0.00079	38.55	8


==> figures/benchmarks/data/iris_np_precise.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
7.1576393699646	0.1437694502629776	0.0	26.49	1.5383761978149417	0.10438179425075061	0.0	7.489999999999998	1.4759425067901608	0.19507299503410797	0.0	5.510000000000002	1
44.942254922389985	0.010684493520346176	1.4000000000000001e-05	60.27	20.41649927854538	0.010681099964856932	1.4000000000000001e-05	27.270000000000003	46.83419547319412	0.06973591920080556	0.000786	88.72999999999999	2
61.680362489223484	0.0028120296159400383	0.0	80.45	28.67117097616196	0.002811330480355807	0.0	33.45	62.83050915956497	0.01972403853621848	0.0	56.55	3
89.91611423254012	0.004390137078881579	4e-06	157.33	61.48519959211349	0.00439013465986181	4e-06	96.33000000000001	239.31013236284258	0.02978506325390513	0.00019600000000000002	375.66999999999996	4
64.82914402961731	1.811939326105618e-05	0.001118	87.94	25.962087898254396	1.809970053533147e-05	0.001118	26.939999999999998	37.007452459335326	9.871002018951934e-05	0.036882	43.06	5
85.25600189685821	0.006876728743155686	0.0	149.03	47.08145231723785	0.006876721027772683	0.0	65.03	107.79299479007722	0.07115144947820284	0.0	235.97	6
3552.9073234272005	5.2795035024586035e-11	0.0002	586.93	3197.245398349762	5.2795034991273714e-11	0.0002	415.92999999999995	28217.089984111786	5.003631753592947e-10	0.0126	1953.0700000000002	7
130.94535375356674	2.8720356813816167e-09	0.0	101.01	51.31399894475936	2.870359806578873e-09	0.0	46.010000000000005	138.08818697214127	1.0204138702764662e-08	0.0	94.99	8


==> figures/benchmarks/data/iris_np_vfast.tex <==
times_mean	volumes_mean	fraction_in_collision_mean	num_faces_mean	times_err_minus	volumes_err_minus	fraction_in_collision_err_minus	num_faces_err_minus	times_err_plus	volumes_err_plus	fraction_in_collision_err_plus	num_faces_err_plus	env
0	0	0	0	0	0	0	0	0	0	0	0	0
0.1682763910293579	0.1560011125128415	0.039628	22.7	0.05041392803192138	0.14483890529160875	0.039628	6.699999999999999	0.28833190441131595	0.29675782886600166	0.247172	9.3	1
0.9938970136642457	0.016840084428766215	0.04037000000000001	41.6	0.5516846704483033	0.016835392742080728	0.04037000000000001	14.600000000000001	1.0634645891189574	0.11025896632384462	0.30002999999999996	43.4	2
1.2266513967514039	0.007835968778277198	0.028517999999999998	51.38	0.739893879890442	0.007834697551403548	0.028517999999999998	21.380000000000003	1.2288458681106567	0.0629651212632965	0.235082	31.619999999999997	3
1.345428216457367	0.008276777011549132	0.067844	77.28	0.9203765273094178	0.008276769394759135	0.067844	39.28	1.6800196290016174	0.07552372574971784	0.273356	95.72	4
1.3165054798126221	2.804875038898052e-05	0.10184999999999997	62.86	0.5022519111633301	2.800536980636276e-05	0.10184999999999997	21.86	0.8679301261901855	0.00020850030558201116	0.7353500000000001	30.14	5
1.5357209706306458	0.01505195697236538	0.09216799999999999	83.99	0.9603117966651917	0.015051944455821803	0.09216799999999999	40.989999999999995	1.8121188616752624	0.16284891968382964	0.484632	85.01	6
20.482455456256865	2.397808419328959e-10	0.060582000000000004	242.05	15.372804844379424	2.397808418106169e-10	0.059982	147.05	73.61794523000717	3.39869202309717e-09	0.49601799999999996	471.95	7
2.2767344760894774	4.798052460109174e-09	0.000684	75.34	0.8876391696929931	4.7963264859451586e-09	0.000684	25.340000000000003	1.1399170112609864	3.047447349120994e-08	0.009715999999999999	25.659999999999997	8


==> figures/benchmarks/multiplot.tex <==
\pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.5ex}}
\pgfplotsset{every x tick label/.append style={font=\tiny, xshift=0.5ex}}

% \begin{tikzpicture}
%      % Legend placed absolutely
%  \begin{scope}[shift = {(0, 0)}]
%     \node at (0,0.0) [scale = 0.8] {%
%         \begin{axis}[
%             hide axis,
%             legend columns=3, % Adjust number of columns if needed
%             legend style={draw=black, fill=white,},
%             xmin=0,
%             xmax=0.1,
%             ymin=0,
%             ymax=0.1,
%         ]
%             \addlegendimage{color=blue, mark=*}
%             \addlegendentry{IrisNP}
%             \addlegendimage{color=red, mark=square*}
%             \addlegendentry{FastIris}
%             \addlegendimage{color=magenta, mark=triangle*}
%             \addlegendentry{RayIris}
%         \end{axis}
%     };
%     \end{scope}
% \end{tikzpicture}
\begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            ylabel={time [s]},
            ymin=0.01,
            ymax=50000,
            ytick = {0.01, 1, 100,10000},
            title = {Fast},
            ymode=log,
         % Adjust this number based on the number of entries
        % draw=black, 
        % anchor=north west,
        % fill=white, 
        % align=left}
        ]
            % \addplot+[blue, only marks, mark options={scale=0.4}, error bars/.cd, y dir=both, y explicit] table[x=x,y=y,y error=y_error] {figures/benchmarks/data/dummy1.dat};
            %\addplot[blue] table[x=env, y=times_mean] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=times_mean,y error plus=times_err_plus, y error minus=times_err_minus] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=times_mean,y error plus=times_err_plus, y error minus=times_err_minus] {figures/benchmarks/data/fast_iris_fast.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            ymin=0.01,
            ymax=50000,
            ytick = {0.01, 1, 100,10000},
            title = {Balanced},
            ymode=log,
        ]
            %\addplot[blue] table[x=env, y=times_mean] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=times_mean,y error plus=times_err_plus, y error minus=times_err_minus] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=times_mean,y error plus=times_err_plus, y error minus=times_err_minus] {figures/benchmarks/data/fast_iris_balanced_3.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            ymin=0.01,
            ymax=50000,
            title = {Precise},
            ytick = {0.01, 1, 100,10000},
            ymode=log,
        ]
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=times_mean,y error plus=times_err_plus, y error minus=times_err_minus] {figures/benchmarks/data/iris_np_precise.tex};
        \end{axis}
    \end{tikzpicture}
    \\
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            %xlabel={$x$},
            ymin=0.0000000000005,
            ymax=1.1,
            ylabel={rel. volume [-]},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            %\addplot[blue] table[x=env, y=volumes_mean] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=volumes_mean,y error plus=volumes_err_plus, y error minus=volumes_err_minus] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=volumes_mean,y error plus=volumes_err_plus, y error minus=volumes_err_minus] {figures/benchmarks/data/fast_iris_fast.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            ymin=0.0000000000005,
            ymax=1.1,
            %xlabel={$x$},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            %\addplot[blue] table[x=env, y=volumes_mean] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=volumes_mean,y error plus=volumes_err_plus, y error minus=volumes_err_minus] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=volumes_mean,y error plus=volumes_err_plus, y error minus=volumes_err_minus] {figures/benchmarks/data/fast_iris_balanced_3.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            %xlabel={$x$},
            ymin=0.0000000000005,
            ymax=1.1,
            ymode=log % Set the y-axis to logarithmic scale
        ]
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=volumes_mean,y error plus=volumes_err_plus, y error minus=volumes_err_minus] {figures/benchmarks/data/iris_np_precise.tex};
        \end{axis}
    \end{tikzpicture}
    \\
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            %xlabel={$x$},
            ymin=0.000001,
            ymax=1.3,
            ylabel={frac. in coll. [-]},
            ytick = {0.000001, 0.0001,0.01,1},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            %\addplot[blue] table[x=env, y=fraction_in_collision_mean] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=fraction_in_collision_mean,y error plus=fraction_in_collision_err_plus, y error minus=fraction_in_collision_err_minus] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=fraction_in_collision_mean,y error plus=fraction_in_collision_err_plus, y error minus=fraction_in_collision_err_minus] {figures/benchmarks/data/fast_iris_fast.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            ymin=0.000001,
            ymax=1.3,
            ytick = {0.000001, 0.0001,0.01,1},
            %xlabel={$x$},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            %\addplot[blue] table[x=env, y=fraction_in_collision_mean] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=fraction_in_collision_mean,y error plus=fraction_in_collision_err_plus, y error minus=fraction_in_collision_err_minus] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=fraction_in_collision_mean,y error plus=fraction_in_collision_err_plus, y error minus=fraction_in_collision_err_minus] {figures/benchmarks/data/fast_iris_balanced_3.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            %xlabel={$x$},
            ymin=0.000001,
            ymax=1.3,
            ytick = {0.000001, 0.0001,0.01,1},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=fraction_in_collision_mean,y error plus=fraction_in_collision_err_plus, y error minus=fraction_in_collision_err_minus] {figures/benchmarks/data/iris_np_precise.tex};
        \end{axis}
    \end{tikzpicture}
    \\
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            %xlabel={$x$},
            ymin=12,
            ymax=10500,
            ylabel={\# faces [-]},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            %\addplot[blue] table[x=env, y=num_faces_mean] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=num_faces_mean,y error plus=num_faces_err_plus, y error minus=num_faces_err_minus] {figures/benchmarks/data/iris_np_vfast.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=num_faces_mean,y error plus=num_faces_err_plus, y error minus=num_faces_err_minus] {figures/benchmarks/data/fast_iris_fast.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            %xlabel={$x$},
            ymin=12,
            ymax=10500,
            ymode=log % Set the y-axis to logarithmic scale
        ]
            %\addplot[blue] table[x=env, y=num_faces_mean] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=num_faces_mean,y error plus=num_faces_err_plus, y error minus=num_faces_err_minus] {figures/benchmarks/data/iris_np_medium.tex};
            \addplot+[red, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=num_faces_mean,y error plus=num_faces_err_plus, y error minus=num_faces_err_minus] {figures/benchmarks/data/fast_iris_balanced_3.tex};
        \end{axis}
    \end{tikzpicture}
    \hspace{-0.25cm}
    \begin{tikzpicture}
        \begin{axis}[
            width=0.35\textwidth,
            height=0.3\textwidth,
            ymin=12,
            ymax=10500,
            %xlabel={$x$},
            ymode=log % Set the y-axis to logarithmic scale
        ]
            \addplot+[blue, only marks, mark options={scale=0.4},error bars/y dir=both, error bars/y explicit] table[x=env,y=num_faces_mean,y error plus=num_faces_err_plus, y error minus=num_faces_err_minus] {figures/benchmarks/data/iris_np_precise.tex};
        \end{axis}
    \end{tikzpicture}

==> figures/irisstepback.tex <==
\begin{tikzpicture}
\draw (-4.4,2.9) -- (-2.8039,3.6907);
\draw  (-2.7986,3.7003) rectangle (-1.2986,3.0003);
\draw  plot[smooth, tension=.9] coordinates {(-2.7986,3.2003) (-2.1247,3.34) (-1.2947,3.15)};
\draw[->] (-2.0936,3.0203) -- (-2.0897,3.34);

\draw[fill,opacity=0.3] (-2.7847,3.525) -- (-1.3097,3.13) -- (-1.2986,3.0003) -- (-2.7986,3.0003)--cycle;
\draw[dashed] (-1.7836,3.0103) -- (-1.7047,3.285);
\draw (-1.3091,3.1752) -- (-2.7992,3.5901);
\draw (-1.7442,3.1101) -- (-1.5392,3.0501) -- (-1.4942,3.2151);
\draw (-3.4,2.5) -- (-1.3,3);


\node at (-1.5,0.3) {$2R$};
\draw[|<->] (-5.2,0.5) -- (1.6,0.5);

\draw[] (-5.2,0.6) -- (-5.2,2);
\draw(1.6,0.4) -- (1.6,2);

%---------------------------------------------
\clip (-5.8,3.3) rectangle + (9.2,-3.);
\draw[dotted, thick]  (-1.8,2) ellipse (3.4 and 3.4);
\draw  (-4,2) ellipse (1.2 and 0.7);

\node at (-3.4,1.8) {$\delta$};
\draw[|<->] (-4,2) -- (-2.8,2);
\draw[|<->] (-4,2) -- (-4,2.7);
\node at (-4.2,2.3) {$\sigma_1$};
\draw[opacity=0.5] (-5.4,2.9) -- (1.6,2) -- (-5.4,1.1);
\draw[fill=gray, opacity = 0.2] (-5.395,1.145) -- (1.6,2) -- (-5.4011,2.8651);

\draw[dashed] (-3.7097,2.7015) -- (-3.8,2) node (v1) {} -- (-3.7116,1.3436);
\draw (v1);
\draw (-3.7405,2.5709) -- (-3.6065,2.5459) -- (-3.5837,2.6618);
\draw (-3.7293,1.4658) -- (-3.6009,1.4771) -- (-3.5839,1.3544);
\draw[|<->] (-4,1) -- (1.6,1);

\node at (-1.5,0.8) {$x$};
\draw[fill=black, opacity=0.5]  plot[smooth, tension=.7] coordinates {(1.7,2.5) (1.6,2.3) (1.6,1.8) (1.8,1.7) (1.7,1.5) (2,1.4) (2.1,1.8) (2,2.1) (1.9,2.5) (1.7,2.5)};
\draw[->]  plot[smooth, tension=.7] coordinates {(0.9,2.8) (1.1,2.3) (1.3,2.5) (1.5739,2.0205)};
\node at (0.8,3) {found collision};
\draw[very thick, teal, opacity = 0.8] (0,2.4) -- (0,1.5);
\draw[<->] (1.6,1.7) -- (0,1.7);
\node at (0.8,1.5) {$\delta$};
\draw (1.6,2) -- (1.6,1.7);
\draw[|<->|] (-0.1113,2.2113) -- (-0.1141,1.7936);
\node at (-0.3,2) {2$l$};

\draw[opacity = 0.8]  (-4.4,2.9) rectangle (-3.4,2.5);



\end{tikzpicture}
